Maximal Violation of Kirchhoff's Law in Planar Heterostructures

Violating Kirchhoff's law has so far required nonreciprocal materials patterned in microstructures. In these configurations, the excitation of a guided or polaritonic mode that lies outside the light cone, often via gratings, was a requirement. Here, we describe how nonreciprocity manifests itself in pattern-free heterostructures. We demonstrate that a resonant mode in a dielectric spacer separating a nonreciprocal film from a back-reflector suffices to maximally violate Kirchhoff's law, and identify the minimal dielectric requirements for such functionality, which are satisfied by currently available materials.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
 
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );
 
        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );
 
        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
 
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
